Revealing the Evolution of Order in Materials Microstructures Using Multi-Modal Computer Vision

The development of high-performance materials for microelectronics, energy storage, and extreme environments depends on our ability to describe and direct property-defining microstructural order. Our present understanding is typically derived from laborious manual analysis of imaging and spectroscopy data, which is difficult to scale, challenging to reproduce, and lacks the ability to reveal latent associations needed for mechanistic models. Here, we demonstrate a multi-modal machine learning (ML) approach to describe order from electron microscopy analysis of the complex oxide La$_{1-x}$Sr$_x$FeO$_3$. We construct a hybrid pipeline based on fully and semi-supervised classification, allowing us to evaluate both the characteristics of each data modality and the value each modality adds to the ensemble. We observe distinct differences in the performance of uni- and multi-modal models, from which we draw general lessons in describing crystal order using computer vision.

==> notused.tex <==
%Text from NeurIPS paper: Akers et al.~developed pyCHIP, a few-shot approach for oversegmentation of STEM images that is robust against noise and requires less data than conventional segmentation methods \cite{akers2021rapid}. In the pyCHIP method, an image is oversegmented into non-overlapping squares, embeddings are extracted from a pretrained classification model and the embeddings of each chip are compared against a small set of hand-selected prototype chips. We note that the unsupervised method discussed in this paper moves beyond pyCHIP, since the present approach does not require labeled data and utilizes a microscopy-specific encoder to compute embeddings. 

%Jiao et al.~performed graph-clustering based unsupervised image segmentation on digital photographs from the BSDS500 and PASCAL VOC 2021 benchmark datasets \cite{jiao2020segmentation}. Images were oversegmented into non-overlapping superpixels (non-rectangular groupings of pixels). Low-level visual features (color, edge, gradient, and image saliency) of each superpixel were fed into an autoencoder to obtain high-dimensional embeddings. A set of similarity scores was computed from the Euclidean distances between embeddings, which were formulated into a similarity graph. Superpixels adjacent in coordinate space were merged if the similarity score fell below a specified threshold. 

%Text from NeurIPS paper: Here, we present a method for the unsupervised segmentation of structural regions within STEM images through the combination of pretrained classification models and graph theory. Embeddings of overlapping superpixels are extracted from a ResNet50 model pretrained on a large dataset of microscopy images \cite{stuckner2022microstructure}. A graph is formed based on the pairwise similarity of the embeddings. The Louvain method \cite{blondel2008fast} is used to identify communities within the graph, which correspond to various structural regions in the material. This approach provides a means to analyze electron microscopy data absent \textit{a priori} knowledge and shows promise to describe order-disorder phase transitions in emerging functional materials.

%%%%%%%%%%%%%%%%%%%%%%%%% INTRO

%Image segmentation aims to partition an image into meaningful regions according to human visual perception, typically based on pre-defined regions in a supervised learning setting. Supervised image segmentation of microscopy data is often limited by its dependence on large annotated datasets. Large-scale efforts have been made in compiling such datasets for specific scenarios. For instance, Stuckner et al.~compiled a large dataset of over 100,000 labeled TEM, SEM, and optical microscopy images of diverse materials and showed that pre-training a segmentation model on this dataset provided improved performance when fine tuning on much smaller task-specific datasets.\cite{stuckner2022microstructure} Relevant to irradiation-induced disorder, Burns et al.~assembled a hand-labeled dataset consisting of 1,000 \textit{in situ} TEM images and trained a segmentation model capable of characterizing irradiation-induced defects in face centered cubic metals.\cite{burns2024deep}

%Despite these efforts, supervised segmentation models struggle to generalize to data that significantly differs from the training data. This generalizability issue has inspired the adoption of learning techniques that require relatively few labeled training examples for the purpose of automatic segmentation and denoising.\cite{kaufmann2021, pelt2018, chen2023small, akers2021rapid} Ideally, these methods leverage a small volume of \textit{a priori} domain knowledge to utilize state-of-the-art segmentation techniques in light of limited training data. %Others are utilizing Bayesian Optimization approaches under the same premise to achieve optimal image analysis workflows that were previously infeasible for manual analysis.\cite{barakati2024physics}  %more citations... 
%\textbf{SARAH: discussion of sparse segmentation methods and your few shot stuff.} %sparse data approaches \cite{chen2023small, akers2021rapid}

%However, in novel scenarios even small data collection can hinder analysis. Therefore, unsupervised approaches are necessary to create a general analysis framework for microscopy data.\cite{shi2022uncovering, williamson2022creating} Previously reported unsupervised approaches for segmenting STEM images often employ statistical clustering methods to some type of descriptor. For instance, Wang et al.~applied principal component analysis (PCA) and k-means clustering on local features obtained from symmetry operations for unsupervised clustering of STEM high-angle annular dark field (HAADF) images.\cite{wang2021segmentation} To identify nanoparticles in STEM images, Wang et al.~applied k-means clustering followed by naive Bayes classification to a set of geometric shape descriptors.\cite{wang2021autodetect}


%Identifying salient features in materials data is a challenging yet important aspect of characterization. Researchers rely on experience and knowledge when analyzing data, often looking for variations in structure and chemical composition, but even the most experienced researchers can struggle to identify subtle differences in both. These difficulties are further compounded in high-throughput settings where time constraints become a factor. Semantic segmentation provides a path towards the automated extraction of salient features, but appropriate data processing is needed to achieve meaningful results.

%%%%%%%%%%%%%%%%%%%%%%%%%

Typically, unsupervised approaches for STEM images have applied statistical clustering methods to some type of descriptor. For instance, Wang et al.~applied principal component analysis (PCA) and k-means clustering on local features obtained from symmetry operations for unsupervised clustering of STEM high-angle annular dark field (STEM-HAADF) images \cite{wang2021segmentation}. To identify nanoparticles in STEM images, Wang et al.~applied k-means clustering followed by naive Bayes classification to a set of geometric shape descriptors \cite{wang2021autodetect}. % unsupervised segmentation in 4D-STEM using unsupervised clustering using non-negative matrix factorization \cite{bruefach2022analysis}

It has been recently shown that the unsupervised segmentation of digital photographs can be achieved by combining image features or learned embeddings and graph theory. Jiao et al.~applied graph clustering to high-dimensional embeddings obtained from an autoencoder fed low-level visual features of color, edge, gradient, and image saliency \cite{jiao2020segmentation}.
%Wang et al.~used graph-cuts on a graph formed from similarities between self-supervised transformer features to perform object localization \cite{wang2022self}. Melas-Kyriazi et al.~performed spectral clustering on a graph Laplacian matrix formed from a combination of color information and unsupervised deep features \cite{melas2022deep}. Aflalo et al.~incorporated node features derived from pre-trained neural networks into the graph and performed clustering using a graph neural network trained on a loss function based on classical graph clustering algorithms \cite{aflalo2022deepcut}. While graph-based image segmentation existed prior to the widespread use of deep-learning-based segmentation \cite{felzenszwalb2004efficient, camilus2012review}, these approaches have not yet been widely applied to electron microscopy data.



% RESULTS AND DISCUSSION

% \begin{figure}[h!]
% \includegraphics[width=\textwidth]{Figures/Figure1-rev1.png}
% \caption{\textbf{Overview of Irradiation Progression}}
% STEM HAADF images of the defect progression under irradiation for each of the initial states.
% \end{figure}
% Figure 1: Overview of progression. Possibly overlaid with few-shot segmentation.

% \begin{figure}[h!]
% \includegraphics[width=\textwidth]{Figures/Figure2-rev1.png}
% \caption{\textbf{Effect of Irradiation on Chemistry}}
% STEM EDS and associated HAADF showing the Fe distribution before and after irradiation in the LFO pristine and LFO defect domains samples. 
% \end{figure}
% Figure 2: Chemical changes from EDS, maybe focusing on a few selected examples.

%\section{Results and Discussion (NeurIPS 2023 Paper)}

%To demonstrate this method, we examine STEM-HAADF images of an epitaxial thin film at three levels of irradiation---0, 0.1, and 0.5 displacements per atom (dpa)---which introduces increasing structural disorder. The single-crystal substrate consists of SrTiO$_3$ (STO), on which a perovskite LaFeO$_3$ (LFO) thin film was grown \cite{taylor2023resolving}. The material was then irradiated to 0.1 and 0.5 dpa, after which a protective Cr cap was sputtered on the film surface. Cross-sectional STEM samples were then prepared, as described in \cite{taylor2023resolving}. The Cr cap is polycrystalline and does not display a lattice structure in the STEM-HAADF image, in contrast to the LFO and STO layers which show clear perovskite lattices prior to irradiation.

%\textbf{Effect of edge weight thresholding}. 
%To reduce connectivity and expose partitions of similar chips, thresholding is applied to the complete graph prior to using the Louvain method. The choice of thresholding value has a noticeable impact on the communities detected by the Louvain method. Because the similarity distribution will be different for each image, we examine a series of thresholding values relative to the distribution: the mean, median, and mode. As demonstrated in Figure \ref{fig:thresholding} of the image prior to irradiation, increasing the thresholding value results in more fine-grained segmentation of the image into the layers visible in the original STEM-HAADF image.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\textwidth]{Figures/LFO-pristine-cutoff.png}
%     \caption{Similarity distribution and segmentation maps for the film prior to irradiation (0 dpa) thresholded at the mean (red), median (green), and mode (blue) of the similarity distribution.}
%     %\vspace{-10pt}
%     \label{fig:thresholding}
% \end{figure}

%Notably, thresholding at the lowest level (the mean) segments the image into two regions: one representing material with a clear crystalline lattice and one representing the chromium cap where no lattice is visible. Increasing the thresholding value from the mean to the median of the similarity distribution leads to segmentation of LFO in the crystalline region. Finally, when increasing the thresholding value from the median to the mode, both the LFO and STO layers as well as the surface are clearly differentiated.

%\textbf{Tracking Irradiation-induced Amorphization}. 
%Irradiation of the surface induces atomic rearrangement with associated loss of crystallinity (amorphization) \cite{spurgeon2020order}, creating an amorphous front that travels further down the lattice with increased irradiation. Figure \ref{fig:LFOpristineirrad} shows the segmentation results for samples irradiated at 0, 0.1, and 0.5 dpa. Edge thresholding was applied at the mode of the corresponding similarity distribution. The segmentation shows a demarcation between the amorphous and crystalline regions. Prior to irradiation, this demarcation relates to the interface between the LFO and the chromium cap. After irradiation, this demarcation follows the line of amorphization in the LFO layer. Amorphous regions in the LFO layer appear as sections of near uniform intensity, indicating a lack of ordered atomic columns. Varying levels of disorder produce images somewhere between the highly ordered atomic columns and completely amorphized regions. Our segmentation method identifies varying levels of amorphization in the LFO layer of samples irradiated to 0.1 and 0.5 dpa.

% \begin{wrapfigure}[22]{r}{0.6\textwidth}
%     \centering
%     \vspace{-4pt}
%     \includegraphics[width=0.6\textwidth]{Figures/LFO-pristine-series-small.png}
%     \vspace{-14pt}
%     \caption{Cross-sectional STEM-HAADF images (top), segmentation maps (middle), and similarity graphs (bottom) for films irradiated to 0 (left), 0.1 (center), and 0.5 dpa (right).}
%     \label{fig:LFOpristineirrad}
% \end{wrapfigure}

%In the irradiated samples, STO does not segment into a single region. We believe this may be an artifact of a loss of focus in the lateral scan direction. Prior to irradiation, the focus is consistent across the image. For the 0.1 dpa sample, the right side of the image is more in focus than the left, and for the 0.5 dpa sample, the left side is more in focus than the right. These minor differences in focus results in slightly reduced similarity values. Notably, the communities comprising the STO layer are tightly integrated in the similarity graphs of the irradiated samples. Therefore, the identification of separate communities in the STO phase may be an artifact of the use of a heuristic algorithm for modularity optimization by the Louvain method.



% CONCLUSIONS

% From neurips paper: Images are oversegmented into overlapping chips, and embeddings for each chip are extracted from a CNN pretrained on a microscopy dataset. A graph is generated based on the similarity of embeddings, to which edge thresholding and the Louvain method are applied. The identified communities represent segmented regions in the image. Notably, we show that our method can be applied to identify irradiation-induced amorphization in atomic-resolution STEM images. Because the resulting similarity scores depend on the encoder from which the chip embeddings are extracted, the use of different encoders will lead to variations in the similarity graph, which could either improve or weaken the segmentation results. In our case, the encoder trained on a microscopy-specific dataset produced effective microstructure feature representations that facilitated the identification of amorphous fronts in STEM images. 

% From neurips paper: As noted in prior work on the segmentation of microscopy data \cite{akers2021rapid}, this approach is sensitive to microscope parameters \cite{sytwu2023generalization}, as well as carbon contamination \cite{lee2022stem}, which must be carefully considered to obtain reliable results. Furthermore, the incorporation of additional modalities has potential to improve classifier performance. For instance, energy-dispersive X-ray spectroscopy (EDS), which identifies elemental species, will aid in the separation of both discrete material layers and amorphized regions subject to radiation-induced segregation.



%\section{Broader Impact (NeurIPS 2023 Paper)}
%Segmentation is a critical step in the determination of structure-property relationships in many important materials and chemical systems. Often, this segmentation is performed by domain experts, limiting throughput and standardization efforts. Present applications of ML in materials characterization problems have typically relied on training neural networks for specific tasks, thus lacking transferability to other tasks. In many instances, there is not enough data to produce reliable training results. Moreover, when there is enough data to train models, it must be painstakingly labeled by a domain expert. 



%If the modalities are combined before classification, then "fusion" is a more appropriate term. If the modalities are combined after classification (individual models are trained separately on different modalities), then "ensemble" is a more appropriate term. I can say that graph clustering (especially how it'll be presented in this paper) is a multimodal fusion technique (more specifically bimodal fusion since we only show HAADF + EDS)




%%Graph clustering of unirradiated and irradiated pristine LFO micrographs results in intelligible segmentation of crystal structure and chemical composition. Before irradiation, the graph clustering method segments the bottom STO layer into two regions. It also identifies an interfacial region between the LFO and chromium cap layers. This is true regardless of the chosen modality as shown in Figure \ref{fig:LFOpristine}. Outliers exist in the LFO and chromium cap layers, but are predominantly found in the chromium cap and segmented interfacial region. All three main layers in the sample can still be identified with clear boundaries drawn between each.

%%After irradiation, using VGG16 image embeddings as input in the unimodal graph clustering method results in segmentation highlighting the differences amongst crystal structure and chemical composition for the STO, LFO, and chromium layers present in the image. The bottom STO layer is no longer segmented into two regions as before. Further, the method no longer detects an interfacial region between the LFO and chromium cap layers. There are also many outliers in the LFO layer. It should be noted that while using this modality can correctly segment the layers present in the image, it continues to incorrectly cluster the irradiation-induced defect pictured in the LFO layer with the STO layer. Raw EDS spectra data is insufficient in picking up the changes in crystal structure due to irradiation but can pick up interfacial regions between both the STO and LFO layers as well as the LFO and chromium cap layers. Combining these two modalities leads to improved segmentation of irradiation-induced disorder. 

%%Agglomerative clustering successfully segments the three layers in the unirradiated case, only picking up on the interfacial region between the LFO and chromium cap layers with the ensemble of VGG16 image embeddings and raw EDS spectra data. In the irradiated case, this method picks up on a fourth region in both unimodal instances. With VGG16 image embeddings, the method segments a scattered region in the LFO layer concentrated near the middle of the layer. With the raw EDS spectra data, the methods segments an interfacial region between the LFO and chromium cap layers. Like the graph clustering method, combining these two modalities leads to improved segmentation of irradiation-induced disorder in the sample. Features from both unimodal segmentation masks are present in the multimodal segmentation mask. The scattered region segmented using VGG16 image embeddings is present, along with the interfacial region identified from the raw EDS spectra segmentation. The unirradiated few-shot results are similar to those from the agglomerative clustering approach with some outliers in the STO layer when using VGG16 image embeddings and the ensemble of VGG16 image embeddings and raw EDS spectra data. The irradiated few-shot results also have outliers in the STO and LFO layers for both inputs. A similar thrid region is identified within the LFO layer when using the ensemble of VGG16 image embeddings and raw EDS spectra data.


%%Looking at the graph and agglomerative clustering results for both the unirradiated and irradiated defect domain LFO micrograph, we see that the contours of the defect region present in the LFO layer is picked up in both the unimodal HAADF and the multimodal combination of HAADF and EDS. Furthermore, the model appears to also pick up on some carbon contamination in the upper right-hand corner of the irradiated sample in both the unimodal HAADF and multimodal combination of HAADF and EDS. The multimodal graph clustering results show a division in the STO layer which is not noticeable to the user. The unimodal EDS graph clustering results show an interfacial region identified between the LFO and STO layers for both unirradiated and irradiated cases. While this is not the case for the agglomerative clustering results, the unimodal EDS and multimodal results for both unirradiated and irradiated cases show the chromium cap as two regions with one bordering the LFO layer.






\begin{table}[htbp]
\caption{Adjusted mutual information score between modalities for pristine STO/LFO sample before and after irradiation.}
\begin{tabular}{lcccccc}
\hline
 & \multicolumn{3}{c}{0 dpa} & \multicolumn{3}{c}{0.1 dpa} \\
 & haadf-eds & haadf-ensemble & eds-ensemble & haadf-eds & haadf-ensemble & eds-ensemble \\
\hline
community detection & 0.61 & 0.86 & 0.69 & 0.55 & 0.73 & 0.74 \\
agglomerative clustering & 0.86 & 0.94 & 0.93 & 0.64 & 0.90 & 0.79 \\
few-shot classification & 0.80 & 0.97 & 0.81 & 0.62 & 0.87 & 0.71 \\
\hline
\end{tabular}
\label{tab:LFOpristine}
\end{table}

\begin{table}[htbp]
\caption{Adjusted mutual information score between modalities for defective STO/LFO samples before and after irradiation.}
\begin{tabular}{lcccccc}
\hline
 & \multicolumn{3}{c}{0 dpa} & \multicolumn{3}{c}{0.1 dpa} \\
 & haadf-eds & haadf-ensemble & eds-ensemble & haadf-eds & haadf-ensemble & eds-ensemble \\
\hline
community detection & 0.48 & 0.48 & 0.5 & 0.57 & 0.65 & 0.68 \\
agglomerative clustering & 0.79 & 0.96 & 0.84 & 0.60 & 0.86 & 0.80 \\
few-shot classification &  0.70 & 0.96 & 0.72 & 0.61 & 0.76 & 0.81 \\
\hline
\end{tabular}
\label{tab:LFOdefect}
\end{table}

==> outline.tex <==
Questions:
What is order?
Effect of uni- vs multi-modal data?

Samples:
1) lfo pristine -- structurally/chemically homogeneous
2) lfo defect   -- structurally/chemically inhomogeneous (iron-rich in defect regions)


Figures:
1) workflow for approach [Sarah]
   -- data modalities -- cluster method -- explainability
2) Grid of data with Bethany's arrows
3) Comparison of methods (two images) [Jenna]
    -- spectrum from unsupervised (graph) -> unsupervised but with clusters (ML) -> lightly supervised (few-shot)
    -- (a prior knowledge) don't know what to expect -> have an idea of how many regions -> have an idea of which regions are which
4) Explanability -- each image, best mode per method [Mike]
    -- post-processing FFT and EDS atom percent
    -- Jenna and Mike discuss which clustering results to use
       same as those used in Fig 3?


Results:
1) Paragraph/sentence on how ML approaches can identify irradiation-induced disorder in pristine material, but fails as describing pre-irradiation disordered regions as well as irradiation-induced disorder
  -- DBSCAN didn't work, kmeans and agglom clustering was similar 
  --- amorphization from irradiation
  --- pre-existing disorder from growth
  -- heavily dependent on choice of number of clusters

2) Unsupervised graph: 

3a) Few-shot mid-fusion: 

3b) Few-shot soft ensemble: 

3c) Few-shot hard ensemble: 
(need to redo 0.1 dpa defect domains with new hdf5s)
   -- in 0dpa-pristine-most disagreement at boundaries
   -- hard ensemble eds spectra/image encoding best for 0.1dpa-pristine
   -- resputter picked up in STO layer in 0.1dpa-defect (image encoding/eds spectra)

3d) Talk about not picking up defects in 0-defect when 3 sets are used
    -- what happens when 4 support sets are used?

Overall)
EDS spectra fusion works better for few-shot
EDS atom percent works better for graph

--- look at hard ensemble image encoding/eds spectra for few-shots

Explainability)
a) FFT -- crystallinity 
b) class region atom percent resumming













1) Join Embeddings
    a) simple concat of embeddings -- the large difference in vector size of different modality embeddings may lead to bias towars the larger embedding
    b) larger embedding reduced to the size of the smaller embedding (rolling sum, etc.) -- may lose fine-grained information in larger embedding

2) Soft Ensemble
    a) few-shot: pass each modality through ProtoNet, average the output class P over all modalities, determine class from max average P
    b) graph: calculate separate normalized similarity scores, average between modalities*, perform Louvain clustering
        * Arman also trying weighting modalities by histogram bin counts
    c) ML: pass each modality separately, average P*, determine class from max average P
        * Limits sklearn methods to those that output P: DBSCAN and HDBSCAN
        * https://scikit-learn.org/stable/modules/classes.html#module-sklearn.cluster
    Caveat: different similarity/probability distributions between modalities lead to uneven weighting/bias

3) Quasi-Hard Ensemble
    a) few-shot:  pass each modality through ProtoNet, assign classes for each modality, use vector of class assignment as class label
    b) graph: pass each modality separately, perform clustering for eahc modality separately, use vector of class assignment as class label
    c) ML: pass each modality separately, assign classes for each modality, use vector of class assignment as class label



